A time and space optimal stable population protocol solving exact majority

We study population protocols, a model of distributed computing appropriate for modeling well-mixed chemical reaction networks and other physical systems where agents exchange information in pairwise interactions, but have no control over their schedule of interaction partners. The well-studied *majority* problem is that of determining in an initial population of $n$ agents, each with one of two opinions $A$ or $B$, whether there are more $A$, more $B$, or a tie. A *stable* protocol solves this problem with probability 1 by eventually entering a configuration in which all agents agree on a correct consensus decision of $\mathsf{A}$, $\mathsf{B}$, or $\mathsf{T}$, from which the consensus cannot change. We describe a protocol that solves this problem using $O(\log n)$ states ($\log \log n + O(1)$ bits of memory) and optimal expected time $O(\log n)$. The number of states $O(\log n)$ is known to be optimal for the class of polylogarithmic time stable protocols that are "output dominant" and "monotone". These are two natural constraints satisfied by our protocol, making it simultaneously time- and state-optimal for that class. We introduce a key technique called a "fixed resolution clock" to achieve partial synchronization. Our protocol is *nonuniform*: the transition function has the value $\left \lceil {\log n} \right \rceil$ encoded in it. We show that the protocol can be modified to be uniform, while increasing the state complexity to $\Theta(\log n \log \log n)$.

==> sections/old-clock-proofs.tex <==

\subsection{Clock synchronization theorem}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/ideal_clock_distribution.pdf}
    \caption{
    A snapshot of the expected distribution of minutes of the fixed-resolution phase clock. 
    {\bf Note:} this is not a discrete simulation, which would be prohibitively expensive for the large values of $n$ required to clearly show this qualitative behavior.
    To get a scale down to these minimal fractions of $10^{-70}$, this plot comes from simulating the ODEs corresponding to the ``clock drip'' and ``clock epidemic'' reactions (line~\ref{line:clock-drip} and line~\ref{line:clock-epidemic} in \phaseMainAveraging).
    With fractions on a log scale, we can clearly see the back tail (towards smaller minutes) of the distribution decaying exponentially and the front of the distribution decaying like $e^{-i^2}$.}
    \label{fig:ideal_clock_distribution}
\end{figure}

\todo{DD: replace~\cref{fig:ideal_clock_distribution} with stochastic simulation now that we have a magic simulator}

\todo{ES: comparison with two choices phase clock. advantages: simpler tail behavior, not necessary to analyze tail to show the decay at the head. parameterized by p, which allows parameter to bring clock into a tighter distribution.}


We will first consider the behavior of the $\roleclock$ agents in \phaseMainAveraging. The goal is to show their $\fieldminute$ fields remain tightly concentrated while moving from $0$ up to $kL$, summarized in Theorem~\ref{thm:clock}. See Figure~\ref{fig:ideal_clock_distribution} for the ideal expected clock distribution. The back tail behind the peak of the $\fieldminute$ distribution decays exponentially, since these agents are brought ahead by epidemic at a constant rate and thus their counts each decay exponentially. The front part of the distribution decays much more rapidly. With a fraction $f$ of agents at $\fieldminute = i$, the rate of the drip reaction is proportional to $f^2$. This repeated squaring leads to the concentrations at the leading minutes decaying like $\exp(-i^2)$. The rapid decay is key to showing that very few $\roleclock$ agents can get very far ahead of the rest.

The analysis will mostly follow the proof structure to the original proofs of this clock in \cite{gasieniec2020time}. Our Lemmas \ref{lem:clock-epidemic}, \ref{lem:clock-lower-bound}, \ref{lem:clock-upper-bound} are variants of their Lemmas 5,6,7.
Our Lemma~\ref{lem:clock-level-gap}, establishing the rapid decay of the front of the distributions that bounds that number of agents at too high of a $\fieldminute$, shows a similar result to their Lemma 4. However, to achieve the requisite probability bounds for Theorem~\ref{thm:clock}, we require careful repeated application of Azuma's inequality and acknowledging that a minute could be ``leaky'', getting its first agents far ahead of the expected distribution, with small but non-negligible probability.

We start by consider an entire population running the clock transitions (lines 1-5 of \phaseMainAveraging), so $|\clocks| = n$. The following lemmas describe the behavior of just this clock protocol. In our actual protocol, the clock agents are a subpopulation $|\clocks| = c \cdot n$, and these clock transitions only happen when two clock agents meet with probability $\binom{|\clocks|}{2}\big / \binom{n}{2}\sim \frac{1}{c^2}$. The main theorem of the section adapts to this general situation and gives the high probability guarantees on the clock behavior.

For each minute $i$ and parallel time $t$, define $c_{\geq i}(t) = |\{c:c.\fieldminute \geq i\}| / |\clocks|$ to be the fraction of clock agents at minute $i$ or beyond at time $t$. Then define $t^{>0}_i = \min\{t:c_{\geq i}(t) > 0\}$, $t^{0.1}_i = \min\{t:c_{\geq i}(t) \geq 0.1\}$ and $t^{0.9}_i = \min\{t:c_{\geq i}(t) \geq 0.9\}$ to be the first times where this fraction becomes positive, hits $0.1$ and hits $0.9$.

We first show that the $c_{> i}$ is significantly smaller than $c_{\geq i}$ while both are still increasing, so the front of the clock distribution decays very rapidly. In our argument, we consider three types of reactions that change the counts at minutes $i$ or above:
\begin{enumerate}[(i)]
    \item \label{rxn:drip} Drip reactions $i,i \to i,(i+1)$ (line~\ref{line:clock-drip} in \phaseMainAveraging)
    \item \label{rxn:i-1epidemic} Epidemic reactions $j,k \to j,j$, for any minutes $j,k$ with $k \leq i < j$ (line~\ref{line:clock-epidemic} in \phaseMainAveraging)
    \item \label{rxn:iepidemic} Epidemic reactions $j,k \to j,j$, for any minutes $j,k$ with $k < i \leq j$ (line~\ref{line:clock-epidemic} in \phaseMainAveraging)
\end{enumerate}
Note we ignore the drip reactions $(i-1),(i-1) \to (i-1),i$, which would only help the argument, but we do not have guarantees on the count at minute $i-1$.


We first reason about how large the count at minute $i$ gets before the first agents make it to minute $i+1$ via reaction \ref{rxn:drip}. For a parameter $\epsilon$ we will set later to $\epsilon = 0.15$, if the first drip reaction \ref{rxn:drip} happens before minute $i$ reaches count $n^\epsilon$, we call $i$ a \emph{leaky} minute. Otherwise, if its count reaches at least $n^\epsilon$ before its first drip reaction \ref{rxn:drip}, we call $i$ a \emph{non-leaky} minute.

If minute $i$ is leaky, we will not be able to reason about the count $c_{> i}$ at minutes $i+1$ and beyond being significantly smaller, because minute $i+1$ got a head start with the early leak reaction. Thus we must consider non-leaky minutes, and bound the probability of such a leak. Crucially, this bound is weaker than the with high probability bound of $O(1/n)$, so we must acknowledge the possibility of one leak happening within a set of consecutive minutes.

\begin{lemma}
\label{lem:clock-early-drip}
For any $0 < \epsilon < 1$, the probability minute $i$ is a leaky minute 
$\Pr[ c_{\geq i}(t^{>0}_{i+1}) < n^\epsilon / n ]
= O(p/n^{1-2\epsilon})$. 
These probabilities are independent across all minutes.
\end{lemma}

\todo{ES: consider effect of requiring a counter before activating a drip reaction, to boost this probability bound}

\begin{proof}
Observe that $t^{>0}_{i+1}$ is the time of the first drip reaction \ref{rxn:drip}. When there are $j$ agents at minute $i$, the probability of reaction \ref{rxn:drip} is $p\binom{j}{2} / \binom{n}{2}$. The probability of epidemic reaction \ref{rxn:iepidemic} increasing the count at minute $i$ is $j(n-j) / \binom{n}{2}$, so the probability reaction \ref{rxn:drip} happens first is at most
\[
\frac{pj(j-1)/2}{j(n-j)+pj(j-1)/2} = \frac{pj-1}{2(n-j)+pj-1} < \frac{pj}{n}.
\]
We can then bound the probability of an early drip that makes $i$ a leaky minute: 
\[
\Pr[ c_{\geq i}(t^{>0}_{i+1}) < n^\epsilon / n ]
\leq 
\sum_{j=1}^{n^\epsilon} \frac{pj}{n} = O(pn^{2\epsilon} / n) = O(p/n^{1-2\epsilon}).
\]
Notice that these probabilities are independent across minutes $i$, since they only depend on comparing times of distinct reactions \ref{rxn:drip} vs \ref{rxn:iepidemic}, and occur on distinct time intervals $(t_i^{>0}, t_{i+1}^{>0})$.
%
% Trying to push this argument longer.
% $n^{\epsilon_0} \leq x \leq n^{\epsilon_1}$.
% Want to say the number of $x$ increases before each $y$ increase is lower bounded by a geometric. Probability of a $y$ increase is $2y(1-y) + px^2 \leq 2y + pn^{2\epsilon_1}$. Probability of an $x$ increase without increasing $y$ is $2(x-y)(1-x) \geq 2(n^{\epsilon_0} - y)(1 - n^{\epsilon_1})$. So we have a geometric with success probability
% \[
% g \leq \frac{2y + pn^{2\epsilon_1}}{2(n^{\epsilon_0} - y)(1 - n^{\epsilon_1}) + 2y + pn^{2\epsilon_1}}
% \]
% which gives
% \[
% \E(\Delta X) \geq 1/g - 1 = \frac{2(n^{\epsilon_0} - y)(1 - n^{\epsilon_1})}{2y + pn^{2\epsilon_1}} \approx \frac{n^{\epsilon_0}}{y}
% \]
% where we assume $y$ is smaller than $n^{\epsilon_0}$ but larger than $pn^{2\epsilon_1}$.
%
% The sum of geometrics as $y$ increases is $\sum_{Y=1}^{\log n} \frac{n\cdot n^{\epsilon_0}}{y}$. This should let us say that $y$ increases to at most $\log n$ before $x$ doubles.
%
% $1\leq j \leq n^{\epsilon_1}$. Here drip probability is $pn^{2\epsilon_1}$. When at count $Y=yn$, the probability of a $y$ epidemic is $2y(1-y)$, so probability of $Geom\qty(\frac{2x(1-x)}{2x(1-x)+px^2+2y(x-y)})-1$
\end{proof}

We can now show that after a non-leaky minute $i$ reaches fraction $c_{\geq i} = 0.1$, the 
fraction
$c_{> i}$ is still sufficiently small.

\begin{lemma}
\label{lem:clock-level-gap}
A non-leaky minute $i < kL$ satisfies $c_{> i}(t_i^{0.1}) \leq 10 \cdot p \cdot 0.1^2 = 0.001$ with very high probability.
\end{lemma}

% \begin{proof}
% $\Phi = \ln(y / x^2) = \ln(y) - 2\ln(x)$.

% $\Delta\Phi_{\Delta y} \sim 1/(yn)$

% $\Delta\Phi_{\Delta x} \sim -2 / (xn)$

% \begin{align*}
%     \E[\Delta\Phi] &= \Pr[\Delta y]\cdot \Delta\Phi_{\Delta y} + \Pr[\Delta x] \cdot \Delta\Phi_{\Delta x} \\
%     &\leq \frac{px^2 + 2y(1-y)}{yn} - \frac{2x(1-x)2}{xn} \\
%     &= \frac{1}{n}[\frac{px^2}{y} + 2(1-0) - 4(1-0.1)] \\
%     &\leq \frac{1}{n}[\frac{px^2}{y} - 1.6]
% \end{align*}

% Azuma's inequality should give WVHP when $\frac{1}{\sum_{i=1}^{\Theta(n\log n)} (1/yn)^2} = \Omega(n^\epsilon)$

% $$
% \frac{1}{\sum_{i=1}^{\Theta(n\log n)} (1/yn)^2} = \frac{y^2 n}{\log n}
% $$

% Need $y = \Omega(n^{-0.5+\epsilon})$, so something like $y = n^{-0.49}$.

% $\Phi = y - cpx^2$.

% $\Delta\Phi_{\Delta y} = 1$

% $\Delta\Phi_{\Delta x} = -cp((x+1)^2 - x^2) = - (2x + 1)cp $

% \begin{align*}
%     \E[\Delta\Phi] &= \Pr[\Delta y]\cdot \Delta\Phi_{\Delta y} + \Pr[\Delta x] \cdot \Delta\Phi_{\Delta x} \\
%     &\leq px^2 + 2y(1-y) - (2x+1)cp(2x)(1-x)
% \end{align*}

% \end{proof}

\begin{proof}
Assume minute $i$ is a non-leaky minute.
We start the argument at time $t_{i+1}^{>0}$, where $c_{> i}(t_{i+1}^{>0}) = 1 / n$ by definition of time $t_{i+1}^{>0}$, and $c_{\geq i}(t_{i+1}^{>0}) \geq n^\epsilon / n = n^{-0.85}$ because minute $i$ is a non-leaky minute.

Define $x = x(t) = c_{\geq i}(t)$ and $y = y(t) = c_{> i}(t)$, and $X = xn, Y=yn$ to be the corresponding counts. Our goal is to show $y \leq 10px^2$, which implies the desired final bound $y(t_i^{0.1}) \leq 10 \cdot p \cdot 0.1^2$. 

% "A" means "the barrier ABOVE i", i.e, from i+1 or above to i or below
% "B" means "the barrier BELOW i", i.e, from i or above to below i
% \newcommand{\downto}[2]{\ensuremath{\qty[\downarrow^{#1}_{#2}]}}
% \newcommand{\downto}[2]{\ensuremath{\qty[{#1} \text{ to } {#2}]}}
\newcommand{\downto}[2]{\ensuremath{\qty[{#1} \to {#2}]}}
\newcommand{\crossA}{\downto{{<}i}{{\geq}i}}
\newcommand{\crossB}{\downto{{\leq}i}{{>}i}}
\newcommand{\crossAandB}{\downto{{<}i}{{>}i}}
\newcommand{\crossAnotB}{\downto{{<}i}{{=}i}}
\newcommand{\crossBnotA}{\downto{{=}i}{{>}i}}

Among the reaction types \ref{rxn:drip}, \ref{rxn:i-1epidemic}, \ref{rxn:iepidemic}, 
we identify events for how $x$ or $y$ can change via an agent changing its minute:
\begin{description}
    \item[$\crossB$:]
    From at most $i$ to beyond $i$, caused by~\ref{rxn:drip} or~\ref{rxn:i-1epidemic}.
    Increases $y$.
    Increases $x$ only if start minute is $< i$.
    \[
    \Pr\crossB = \Pr[ \text{\ref{rxn:drip}} ] + \Pr[ \text{\ref{rxn:i-1epidemic}} ] \sim p(x-y)^2 + 2y(1-y) \leq px^2 + 2y(1-y)
    \]
    
    \item[$\crossA$:]
    From before $i$ to at least $i$, caused by~\ref{rxn:iepidemic}.
    Increases $x$.
    Increases $y$ only if final minute is $> i$.
    \[
    \Pr\crossA \sim 2x(1-x)
    \]
    
    \item[$\crossAandB$:]
    From before $i$ to beyond $i$, caused by~\ref{rxn:i-1epidemic} $\cap$ \ref{rxn:iepidemic}.
    Increases $x$ and $y$.
    \[
    \Pr\crossAandB\sim 2y(1-x)
    \]
    
    \item[$\crossAnotB$:]
    From before $i$ to exactly $i$, caused by~\ref{rxn:iepidemic} $\setminus$ \ref{rxn:i-1epidemic}.
    Increases $x$ but not $y$.
    \[
    \Pr\crossAnotB\sim 2(x-y)(1-x)
    \]
    
    \item[$\crossBnotA$:]
    From exactly $i$ to beyond $i$, caused by~\ref{rxn:drip} or 
    \ref{rxn:i-1epidemic} $\setminus$ \ref{rxn:iepidemic}.
    Increases $y$ but not $x$.
    \[
    \Pr\crossBnotA \leq px^2 + 2y(x-y)
    \]
\end{description}


To analyze how these reactiosn affect the changing relationship between $x$ and $y$, we will use the continuous piecewise potential function
\[
\Phi = \Phi(t) =
\begin{cases}
\Psi = \ln(y / 10px^2) = \ln(y) - 2\ln(x) - \ln(10p) &\mbox{if }
y > 10px^2
\\
\Gamma = y - 10px^2 &\mbox{if } y \leq 10px^2.
\end{cases}
\]
Note that $\Psi \geq 0$, $\Gamma \leq 0$, and the desired inequality becomes $\Phi \leq 0$ corresponding to the domain of $\Gamma$. The potential $\Phi$ is designed to be a supermartingale, whose decreasing tendency reflects the fact that the system evolves to bring $y$ below $10px^2$.

Our initial condition is $x = x(t_{i+1}^{>0}) \geq n^{\epsilon - 1}$ and $y = y(t_{i+1}^{>0}) = n^{-1}$, where we have
\[
\Phi(t_{i+1}^{>0}) \leq \ln(n^{-1}) -2\ln(n^{\epsilon - 1}) - \ln(10p) \sim (1-2\epsilon)\ln n = 0.7\ln n.
\]

Increasing $y$ changes $\Phi$ by
\[
\Delta\Phi_{\Delta y} =
\begin{cases}
\Delta\Psi_{\Delta y}  = \ln\qty(y+1/n) - \ln(y) = \ln\qty(1+1/(yn)) \sim 1/(yn) &\mbox{if } y > 10px^2
\\
\Delta\Gamma_{\Delta y}  = y+1/n - y = 1/n &\mbox{if } y \leq 10px^2.
\end{cases}
\]
% This change $\Delta y$ happens via reactions \ref{rxn:drip} and \ref{rxn:i-1epidemic},
% \dd{event $\crossB$,} with probabilities 
% $\Pr[ \text{\ref{rxn:drip}} ] \sim p(x-y)^2 \leq px^2$ 
% and 
% $\Pr[ \text{\ref{rxn:i-1epidemic}} ] \sim 2y(1-y)$,
% \dd{so $\Pr\qty[\crossB] \sim px^2 + 2y(1-y)$.}

Increasing $x$ changes $\Phi$ by 
\[
\Delta\Phi_{\Delta x}  =
\begin{cases}
\Delta\Psi_{\Delta x} = -2\ln(x+1/n) + 2\ln(x) = -2\ln\qty(1+1/(xn)) \sim -2/(xn) &\mbox{if } y > 10px^2
\\
\Delta\Gamma_{\Delta x} = -10p(x+1/n)^2 + 10px^2 \sim -20px/n &\mbox{if } y \leq 10px^2.
\end{cases}
\]
% This change $\Delta x$ happens via reaction \ref{rxn:iepidemic},
% \dd{event $\crossA$,}
% with probability 
% $\Pr[ \text{\ref{rxn:iepidemic}} ] \sim 2x(1-x)$,
% \dd{so $\Pr\qty[\crossA] \sim 2x(1-x)$}.

% Note also that an interaction could count as both reaction \ref{rxn:i-1epidemic} and \ref{rxn:iepidemic} with probability 
% $\Pr[ \text{\ref{rxn:i-1epidemic}} \cap \text{\ref{rxn:iepidemic}} ] \sim 2y(1-x)$, 
% so 
% $\Pr[ \text{\ref{rxn:i-1epidemic}} \setminus \text{\ref{rxn:iepidemic}} ] \sim 2y(x-y)$ 
% and 
% $\Pr[ \text{\ref{rxn:iepidemic}} \setminus \text{\ref{rxn:i-1epidemic}} ] \sim 2(x-y)(1-x)$.

% \textcolor{red}{If we also tried to include drip reactions into $x$, they have probability $\Pr < x / r$ if we could inductively assume the same distribution for $c_{\leq(i+1)}$ and $x$. The effect of using this term is shown in red.}

Our proof strategy will be to use Azuma's Inequality (Theorem~\ref{thm:azuma}) on this supermartingale $\Phi$ in order to show the desired inequality holds. A key difficulty will be controlling the bounded differences, where the bound $|\Delta\Phi| \leq \frac{1}{yn}$ is largest for small values of $Y$. If we simply defined the sequence of values of $\Phi$ at each successive interaction, this would be a supermartingale, but every step would have the worst case bound where $Y=1$ and $|\Delta\Phi| \leq 1$. By assuming this worst case where $Y$ is small and $\Delta\Phi$ has very high variance, the result of Azuma's Inequality will be too weak.

To handle this difficulty, we will track the value of $Y$ as it increases from $1$ to $0.1pn$. Our supermartingale $(\Phi_j)_{j=1}^{0.1pn}$ will consistent of the values of $\Phi$ each time that $Y$ increases by 1. This way the difference bound $|\Phi_{j+1} - \Phi_j| \leq \frac{1}{yn} = \frac{1}{j}$ gets tighter as the index $j$ representing the count $Y$ increases.

Define $t_j = \min\{t:Y(t)=j\}$ and $\Phi_j = \Phi(t_j)$ to be the value of $\Phi$ when $Y$ reaches count $j$, so $\Phi_1 = \Phi(t_{i+1}^{>0}) \leq (1-2\epsilon)\ln n = 0.7\ln n$. Our goal is to show $\Phi_{0.1pn} \leq 0$. This will imply that when $Y$ would reach $0.1pn$ at time $t_{0.1pn}$, because $y \leq 10px^2$, we must already have $x \geq 0.1$. Thus the actual time when $x$ reaches $0.1$, $t_i^{0.1} < t_{0.1pn}$.

To compare $\Phi_{j+1}$ to $\Phi_j$, we must track the number of times $X$ changes between $t_{j+1}$ and $t_j$, which will be the random variable $\Delta X_j$. We must consider the number of times event $\crossA$ increases $X$
(a ``failure'')
before event $\crossB$ increases $Y$
(a ``success'')
\footnote{
    Note that we are using the terminology ``success'' in the context of geometric random variables, although an early ``success'' here is bad for the proof. 
    The goal of this proof is to show that $X$ increases many times before $Y$ does, i.e., we would like to show that there are many failures before the first success.
}.
Here we consider a geometric random variable $G_j$ with success probability 
\[
s_j = \frac{
    \Pr \crossB 
}{
    \Pr[ \text{\ref{rxn:drip}} \cup \text{\ref{rxn:i-1epidemic}} \cup
    \text{\ref{rxn:iepidemic}}]
}
=
\frac{
    \Pr \crossB 
}{
    \Pr \crossBnotA
    + \Pr \crossA
}
\leq \frac{px^2 + 2y(1-y)}{px^2 + 2y(x-y) + 2x(1-x)},
\]
where $x = x(t_j), y = y(t_j)$ are the fractions at time $t_j$. 
Note that actually $x$ is increasing between time $t_j$ and $t_{j+1}$, 
so the geometric random variable $G_j$ is assuming that the new agents to minute $i$ are not themselves participating in reactions \ref{rxn:drip} and \ref{rxn:iepidemic}. 
But since $x\leq 0.1$, 
epidemic reaction \ref{rxn:iepidemic} further increasing the value of $x$ is more likely than \ref{rxn:drip} increasing the value of $y$, so this assumption will give a lower bound for the true change $\Delta X_j$, which stochastically dominates $G_j$.

Note that the success event $\crossB = \crossAandB \cup \crossBnotA$ can happen in two disjoint ways.
Our lower bound for $\Delta X_j$ will be $G_j$ if the success event $\crossAandB$ increases the count of both $X$ and $Y$, but $G_j - 1$ if the success event $\crossBnotA$ only increases $Y$. The relative probability of the latter event conditioned on success is
\[
d_j = \frac{\Pr\crossBnotA}
{\Pr\crossB}
= \frac{px^2 + 2y(x-y)}{px^2 + 2y(1-y)}
\]
So $\Delta X_j$ dominates the following random variable:
the geometric $G_j$ 
(with $\E[G_j] = \frac{1}{s_j}$),
then subtracting 1 with probability $d_j$.
We can then bound the expected number of $X$ increases
\[
\E[\Delta X_j] 
\geq 
%(1 - d_j) \cdot \frac{1}{s_j} + d_j \cdot \qty( \frac{1}{s_j} - 1)
%=
\frac{1}{s_j} - d_j 
=
\frac{\Pr\crossA}{\Pr\crossB}
= \frac{2x(1-x)}{px^2 + 2y(1-y)}
\geq \frac{1.8x}{px^2 + 2y}.
\]

We can now analyze the change
$
\Phi_{j+1}-\Phi_j
 = (\Delta\Phi_{\Delta y}) + (\Delta\Phi_{\Delta x})(\Delta X_j)
$, in the two possible cases for the piecewise potential, where either $y > 10px^2$ and $\Phi_j = \Psi_j > 0$ or $y \leq 10px^2$ and $\Phi_j = \Gamma_j \leq 0$. In the first case where $y > 10px^2$, we can bound 
$\E[\Delta X_j]
\geq \frac{1.8x}{px^2 + 2y}
\geq \frac{1.8x}{y/10 + 2y}$ and
\begin{align*}
\E[ \Phi_{j+1}-\Phi_j ] 
= (\Delta\Psi_{\Delta y}) + (\Delta\Psi_{\Delta x})\E[\Delta X_j]
& \leq
\frac{1}{yn} - \frac{2}{xn} \cdot \qty( \frac{1.8x}{2.1y} )
 \leq
\frac{1}{yn} - \frac{1.71}{yn}
=
- \frac{0.71}{j}.
\end{align*}

In the second case where $y\leq 10px^2$, we can bound 
$\E[\Delta X_j]
\geq \frac{1.8x}{px^2 + 2y}
\geq \frac{1.8x}{px^2 + 20px^2}$ and
\begin{align*}
\E[ \Phi_{j+1}-\Phi_j ] 
= (\Delta\Gamma_{\Delta y}) + (\Delta\Gamma_{\Delta x})\E[\Delta X_j]
\leq
\frac{1}{n} - \frac{2rpx}{n} \cdot \qty( \frac{1.8x}{21px^2} )
\leq
\frac{-0.71}{n}.
\end{align*}

To later apply Azuma's Inequality, we will also have to bound the absolute difference $|\Phi_{j+1}-\Phi_j|$.
To handle the technical issue that the above calculations rely on the unbounded geometric random variable $G_j$, we will instead use a truncated geometric $\hat{G}_j = \min(G_j, \frac{11}{s_j})$, which gives a further lower bound for the true change $\Delta X_j$. This has a negligible effect on the mean, since
\[
\E[\hat{G}_j] = \sum_{m = 1}^\infty \Pr[\hat{G}_j \geq m] = \sum_{m=1}^{11/s_j}(1-s_j)^{m-1} = \frac{1 - (1-s_j)^{11 / s_j}}{1-(1-s_j)} = \frac{1}{s_j}\qty(1-e^{-11}).
\]
Then the calculations above change by only a negligible constant which does not change the final bounds. Formally, our supermartingale $(\Phi_j)_{j=1}^{0.1pn}$ will depend on the bounded random variable $\Delta \hat{X}_j$ with $\E[\Delta \hat{X}_j] = \frac{1.8x(1-e^{-11})}{px^2 + 2y}$, which is stochastically dominated by the true change $\Delta X_j$. Since $|\hat{G}_j| \leq 11\E[G_j]$, this implies $|\Delta \hat{X}_j| \leq 11|\E[\Delta \hat{X}_j]|$. We can now bound the absolute difference
\[
|\Phi_{j+1}-\Phi_j| \leq |\Delta\Psi_{\Delta x}|\cdot |\Delta \hat{X}_j| \leq \frac{2}{xn}\cdot 11\qty[\frac{1.8x}{px^2 + 2y}]
\leq \frac{2}{n}\cdot\qty[\frac{20}{2y}]
\leq \frac{20}{yn} = \frac{20}{j}.
\]

% \todo{DD: explain the difficulty with doing the standard Azuma machinery at this point, namely that we have two different bounds on the step-wise potential change $\Phi_{j+1} - \Phi_j$, depending which piece of the piecewise potential we're in, and which piece we're in is itself a r.v., so we can't write a simple sum of the expected changes in potential.}

The remaining technical difficulty in applying Azuma's Inequality is handling the piecewise nature of the potential $\Phi$. We cannot simply sum the expected changes, and must acknowledge that the stronger drift bound $\E[\Phi_{j+1}-\Phi_j] \leq -\frac{0.71}{j}$ only applies when $\Phi > 0$. In order to show the $\E[\Phi]$ drops below $0$ as desired, we will use induction to prove the following bound on the expected potential change as $Y$ ranges between arbitrary values $a$ and $b$:

\[
\E[\Phi_b | \Phi_a] \leq \max\qty(\Phi_a - \sum_{j=a}^{b-1} \frac{0.71}{j}, 0).
\]

% \[
% \E[\Phi_{Y+1} - \Phi_{Y}] \leq 
% \begin{cases}
% \frac{-0.71}{Y}\mbox{ if }
% \Phi_{Y} > 0
% \\
% \frac{-0.71}{n}\mbox{ if }
% \Phi_{Y} \leq 0
% \end{cases}
% \]

We argue by induction on $b$, where the base case $b=a$ is immediate.
For the induction step we use
\[
\E[\Phi_{b+1}|\Phi_b] \leq 
\begin{cases}
\Phi_b-\frac{0.71}{b}\mbox{ if }
\Phi_{b} > 0
\\
\Phi_b-\frac{0.71}{n}\mbox{ if }
\Phi_{b} \leq 0
\end{cases}
\leq
\max\qty(\Phi_b-\frac{0.71}{b}, 0),
\]
and the induction hypothesis for $\E[\Phi_b|\Phi_a]$ to show
\[
\E[\Phi_{b+1}|\Phi_{a}] = \E\bigg[\E[\Phi_{b+1}|\Phi_b]\bigg|\Phi_a\bigg] \leq \max\qty(\E[\Phi_b|\Phi_a] -\frac{0.71}{b}, 0)
\leq \max\qty(\Phi_a - \sum_{j=a}^{b-1} \frac{0.71}{j} - \frac{0.71}{b}, 0).
\]

Now we can finally apply Azuma's Inequality to our supermartingale $(\Phi_j)_{j=1}^{0.1pn}$. We will do it in two stages, first handling the higher variance side where $j \leq \sqrt{n}$ and the deviation bound on $\Phi$ will be $O(\log n)$, then the lower variance side where $j > \sqrt{n}$ and our deviation bound will be $O(1)$.
We will first consider $Y$ ranging across the values $j=1, \ldots, \sqrt{n}$. Using the initial value $\Phi_1 \leq 0.7\ln n$, we have the bound 
\[
\E[\Phi_{\sqrt{n}}] = \E[\Phi_{\sqrt{n}}|\Phi_1] \leq \qty(0.7\ln n - \sum_{j=1}^{\sqrt n -1} \frac{0.71}{j}) \sim 0.7\ln n - 0.71\ln(\sqrt{n}) = 0.345\ln n.
\]
Now we apply Azuma's Inequality (Theorem~\ref{thm:azuma}), with the difference bounds $|\Phi_{j+1}-\Phi_j|\leq \frac{20}{j}$, to conclude
\[
\Pr\big[ (\Phi_{\sqrt{n}} - \Phi_1) - \E[\Phi_{\sqrt{n}} - \Phi_1] \geq \delta] \leq \exp(-\frac{\delta^2}{2\sum_{j=1}^{\sqrt{n}} (\frac{20}{j})^2}).
\]
Taking $\delta = 0.001\ln n$, this implies $\Phi_{\sqrt{n}} \leq \E[\Phi_{\sqrt{n}}] + 0.001\ln n = 0.346\ln n$ with very high probability $1-\exp(-\Theta(\log^2 n)) = 1 - O(n^{-\omega(1)})$.

Next we consider the values $j = \sqrt{n} + 1, \ldots, \alpha n$ for a small linear constant $\alpha = 0.01 p$, where
\[
0.346\ln n - \sum_{j=\sqrt{n}}^{\alpha n-1} \frac{0.71}{j} 
\sim 
0.346\ln n - 0.71(\ln{\alpha n} - \ln{\sqrt n})
\sim
-0.009\ln n < 0,
\]
so from the inductive bound we have
\[
\E[\Phi_{\alpha n}|\Phi_{\sqrt{n}}\leq 0.346\ln n] \leq \max\qty(0.346\ln n - \sum_{j=\sqrt{n}}^{\alpha n-1} \frac{0.71}{j}, 0) = 0.
\]
The remaining values are $j = \alpha n + 1, \ldots, 0.1pn$. Here we use the worst-case bound $\E[\Phi_{j+1}-\Phi_j] \leq \frac{-0.71}{n}$ to conclude $\E[\Phi_{0.1pn} - \Phi_{\alpha n}] \leq \frac{-0.71}{n}\cdot 0.09pn \leq -0.06p$. Now the final bound $\E[\Phi_{0.1pn}|\Phi_{\sqrt{n}}\leq 0.346\ln n] \leq -0.06p$ is at most a small constant below $0$.

A second application of Azuma's Inequality (Theorem~\ref{thm:azuma}) shows
\[
\Pr\big[ (\Phi_{0.1pn} - \Phi_{\sqrt n}) - \E[\Phi_{0.1pn} - \Phi_{\sqrt n}] \geq \delta] \leq \exp(-\frac{\delta^2}{2\sum_{j=\sqrt{n}}^{0.1pn} (\frac{20}{j})^2}).
\]
The sum $\sum_{j=\sqrt{n}}^{0.1pn} (\frac{20}{j})^2 \sim \int_{\sqrt{n}}^{0.1pn} (\frac{20}{j})^2 dj = \Theta(\frac{1}{\sqrt{n}})$. Thus we can set $\delta = 0.06p$ to be a constant, to conclude that $\Pr[\Phi_{0.1pn} \geq 0] \leq \exp(-\Theta(\sqrt{n}))$. Therefore, with very high probability, $\Phi_{0.1pn} < 0$, which implies that $x$ reached the fraction $0.1$ before $y$ reached the fraction $0.1pn$.
\end{proof}
%%%
% These changes give
% \begin{align*}
% \E[ \Delta\Phi ]
% &\leq [\textcolor{red}{x/r} + 2x(1-x)]\cdot [-2/(xn)] + [px^2 + 2y(1-y)] \cdot [1/(yn)]
% \\
% & \leq \frac{1}{n}[\textcolor{red}{-2/r}-4(1-x) + px^2/y + 2(1)]
% \\
% & = \frac{1}{n}[\textcolor{red}{-2/r}- 2 + 4x + px^2/y].
% \end{align*}

% Try another potential $\Gamma = \Gamma(t) = y - x^2 \cdot r \cdot p$, so the desired inequality here is simply $\Gamma \leq 0$.
% \begin{align*}
% \E(\Delta\Gamma) &\leq [2x(1-x)]\cdot [-2xrp/n] + [px^2 + 2y(1-y)] \cdot [1/n]
% \\
% & \leq
% \frac{1}{n}[-4(1-x)prx^2 + px^2 + 2y]
% \\
% & \leq
% \frac{1}{n}[2\Gamma -px^2(2r(1-2x) - 1)]
% \end{align*}

% Want to have the first part of the argument get us down to $\Gamma = -r x^2 p$.

% Want $-2 + 4x + 1/r < constant$ to have drift stay negative, which bounds how large $x$ can be.

% Here we compute the expected change to $\Phi$ during the time when $x$ increases by 1:
% \begin{align*}
% \E[ \Phi(x+1/n)-\Phi(x) ] 
% & \leq
% \frac{-2}{xn}+\frac{y}{x}\cdot \frac{1}{yn} + 
% \E\qty[ Geom\qty(\frac{2x(1-x)}{2x(1-x)+px^2+2y(x-y)})-1] \bigg/ (yn)
% \\
% & \leq
% \frac{-2}{xn}+\frac{y}{x}\cdot \frac{1}{yn} + 
% \E\qty[ Geom\qty(\frac{2x(1-x)}{2x(1-x)+px^2+2(x/2)(x-(x/2))})-1] \bigg/ (rpx^2n)
% \\
% & = \frac{-1}{xn} + \frac{(p+1/2)x^2}{2x(1-x)rpx^2n}
% = \frac{1}{xn}\qty[-1 + \frac{p+1/2}{2r(1-x)p}]
% % \\
% % & \leq \frac{-1}{xn} + \frac{1/r + 2x}{2x(0.9)n}
% % = \frac{-1 + 1/(1.8r)}{xn}+\frac{1}{0.9n}
% \end{align*}
% \todo{ES: bound these changes by sums of random variables, figure out how to give them large deviation bounds}


% Now while $y \geq rpx^2$, we have $px^2 / y \leq 1/r$. We will consider interactions where $x$ or $y$ change via reactions \ref{rxn:drip},\ref{rxn:i-1epidemic},\ref{rxn:iepidemic}, with happen with probability 
% $\Pr[ \Delta x, \Delta y ] = 
% (px^2 + 2y(x-y) + 2x(1-x) + \textcolor{red}{x/r})$.

% Given such an interaction, and using bounds $(2(0.9) + p)x \leq \Pr[\Delta x, \Delta y] \leq (px^2 + 2(x/2)(x-(x/2)) + 2x) = (2.5+p+\textcolor{red}{1/r})x$, we have
% \[
% \E[ \Delta\Phi | \Delta x, \Delta y, y \geq rpx^2 ] \leq \frac{\textcolor{red}{-2/r}- 2 + 4x + 1/r}{n \Pr[ \Delta x, \Delta y ]}
% \leq -\frac{\textcolor{red}{2/r} + (2 - 1/r)}{(2.5+p)nx} + \frac{3}{n}.
% \]

% \begin{align*}
% E(\Delta\Phi | \Delta x, \Delta y) 
% \cdot 
% (px^2 + 2y(1-y) + 2x(1-x))
% &= [\textcolor{red}{x/r} + 2x(1-x)]\cdot -2\log(\frac{x+1/n}{x}) + [px^2 + 2y(1-y)]\log(\frac{y+1/n}{y})
% \\
% & = [\textcolor{red}{x/r} + 2x(1-x)]\cdot -2\log(1 + \frac{1}{xn}) + [px^2 + 2y(1-y)]\log(1+\frac{1}{yn})
% \\
% & \leq [-\textcolor{red}{x/r}-4x(1-x)](1/xn) + [px^2 + 2y](1/yn)
% \\
% & = \frac{1}{n}[-\textcolor{red}{1/r}-4(1-x) + px^2/y + 2]
% \\
% E(\Delta\Phi | \Delta x, \Delta y) 
% \cdot 
% (4+p)x
% & \leq \frac{1}{n}[-\textcolor{red}{1/r} -2 + 4x + 1/r]  \text{ when } y > rpx^2
% \\
% E(\Delta\Phi | \Delta x, \Delta y) 
% &\leq \frac{-2+1/r-\textcolor{red}{1/r}}{(4+p)nx} + \frac{1}{n}
% = \frac{-q}{X} + \frac{1}{n}
% \end{align*}

% Letting $q = \frac{2 - 1/r}{2.5 + p}$, we have $q \geq 0.75$ with $p = 1/100, r = 10$. (Instead letting $p = r = 1$ we would get $q \geq 0.28$).

% Now we consider just the contributions from the $0.1n - n^\epsilon$ times we know $\Delta x$ must happen to bring the count $X=xn$ from $n^\epsilon$ up to $0.1n$, and bound the expected change in potential from these interactions.
% \todo{ES: For this calculation, include the guaranteed interactions when x hits every known value, then also include $O(n \log n)$ other reactions where we don't know what $x$ is, and just know that we have a supermartingale.}
 
% \begin{align*}
%  E(\Phi(t_i^{0.1})-\Phi(t_{i+1}^{>0}))
%  &\leq \int_{n^{\epsilon}}^{0.1n} \frac{-q}{X}+\frac{2}{n} dX
%  \leq
% -q[\ln X]_{n^{\epsilon}}^{0.1n}+0.2
% \\
%  &=
% -q[\ln n + \ln 0.2 - \epsilon\ln n]+0.2 = -q(1-\epsilon)\ln n + q\ln(10) + 0.2.
% \end{align*}

% Then we would have $E(\Phi(t_i^{0.1})) < 0$ when $(1-2\epsilon)\ln n -q(1-\epsilon)\ln n + q\ln(10) + 0.2 < 0$, so we need $1 - 2\epsilon - q(1-\epsilon) < 0$ or $\epsilon > (1 - q) / (2 + q)$. Using $q = 0.52$ gives $\epsilon \approx 0.19$.
% Using $q = 0.2$ gives $\epsilon \approx 0.36$.
% These correspond to error probabilities $1/n^{0.62}$ and $1/n^{0.28}$ from Lemma~\ref{lem:early-drip}.

% $|\Delta\Phi| < O(\frac{1}{yn})$ is the bound for Azuma's inequality.
% For the sum across $x$, we have $1/rpx^2 n$ as the bound, so the bound 
% \[
% \sum_k c_k^2 = \sum_{X={n^\epsilon}}^{0.1n} \qty(\frac{n}{rpX^2})
% \]
% \todo{ES: We need the sum of the bounded differences to be sufficiently small. If we naively take $yn = O(1)$ this will not work.}


% \begin{proof}
% Try to show that the tight inequality $c_{> i} < c_{\geq i}^2 \cdot p \cdot 10$ holds for $n^{-1/4 - \epsilon} < c_{\geq i} < 0.1$. Go inductively by minute, so we can assume it holds for $c_{\leq (i+1)}$. So when $c_{\leq (i+1)} = n^{-1/4}$, we have $c_{\geq i} \leq n^{-1/2}$. Thus when $c_{\geq i} = n^{-1/2}$, we can say $c_{\leq(i+1)} \geq n^{-1/4}$.

% Start when count at minute $i$ is $0$. We don't have to show anything holds until we reach the point where $c_{\geq i} > 1 / \sqrt{n}$ (its count is above $\sqrt{n})$.

% Hypothetical bad case. Count at minute $i$, $C_i = \sqrt{n}$, so $c_i = \sqrt{n} / n = n^{-1/2}$. Count at minute $i-1$, $C_{i-1} = n^{1/4}$, so $c_{i-1} = n^{-3/4}$. So it's not true that $c_{i-1} < c_i^2$. So now the goal is to show that by the time $C_i = n^{3/4}$, the count $C_{i-1} < n^{1/2}$.

% \end{proof}

% \begin{proof}
% Second sketch of a martingale argument:

% Define $x = c_{\geq i}$ and $y = c_{> i}$. Want $y < q x^2$, to eventually show when $x=0.1$, we have $y < 0.01$.

% Probability of $y$ having epidemic $< 2y$. Probability of $x$ drip = $p x^2$.

% Define the $\Phi = \Phi(t) = \frac{y}{x^2}$. Goal is to have $\Phi < q$ or $\Phi < q \cdot p$.

% $E(\Phi(t + \frac{1}{n}) - \Phi(t)) = \ldots \leq \frac{1}{n}[p - \Phi(t)\frac{x-y}{x}]$.

% Could we say something like $y < \frac{x}{2}$.

% Take $x = n^{-3/4}$ and $y=1/n$, $\Phi = n^{1/2}$.
% $E(\Phi(t + \frac{1}{n}) - \Phi(t)) \approx n^{-1/2}$.

% \end{proof}

% \begin{proof}
% Try the base case. Want to show $c_{(L-2)^-}(t_{L-1}^{0.1}) < 0.001$. In other words, wait until minute $L-1$ gets fraction $0.1$ of agents. How many should be at $L-2$?

% This takes $\approx 0.1n$ interactions. The number of drip reactions to minute $L-2$ is at most $0.1n \cdot (0.1)^2 = 0.001n$. The number of epidemic reactions with minute $L-2$ is about $0.001 \cdot 0.1n = 0.0001n$. Thus $c_{(L-2)^-}(t_{L-1}^{0.1}) < 0.0011$.
% (This is base case argument assuming $p=1$.

% Now try for an inductive step. We have $c_{\geq i} = 0.1$ and $c_{> i} < 0.0011$.



% First consider the first agent to arrive at minute $i$. Now wait for the epidemic to get to a certain value, and bound the number of drip reactions that happen at minute $i$. Then we have epidemics at minutes $i-1$ and $i$ racing, and by the time the $i$ epidemic reaches $0.1$, the $i-1$ epidemic has not gotten far.

% Time for the epidemic to hit count $x$: $\ln x$. Let $x = n^\epsilon$, so time to hit $x$ is $\epsilon \ln n$.
% Chance of drip reaction = $p \cdot n^{2\epsilon} / n^2$. Expected number of drip reactions in $p\epsilon n \ln n$ interactions = $p n^{2\epsilon}\cdot \epsilon n\ln n / n^2 = p \epsilon n^{2\epsilon}\ln n / n$.

% minute $i+1$ just hit $n^{1/4}$. Probability of any at minute $i$ = $1/\sqrt{n}$.
% \end{proof}
%%%

Since the previous lemma gives us an upper bound on the count $c_{>i}$ at time $t_i^{0.1}$, we can use this to get a lower bound on the time until $t_{i+1}^{0.1}$ when $c_{>i}$ reaches $0.1$.
\begin{lemma}
\label{lem:clock-lower-bound}
If minute $i$ is non-leaky, then $t_{i+1}^{0.1} - t_{i}^{0.1} \geq 1.48$ with very high probability.
\end{lemma}

\begin{proof}
We start at time $t_i^{0.1}$, where by Lemma~\ref{lem:clock-level-gap} we have $c_{> i}(t_i^{0.1}) \leq 0.1p$ with very high probability.

Define $x = x(t) = c_{\geq i}(t)$ and $y = y(t) = c_{> i}(t)$.
The number of interactions for $Y = yn$ to increase by $1$ is a geometric random variable with mean $\frac{1}{\Pr[\text{\ref{rxn:drip}}] + \Pr[\text{\ref{rxn:i-1epidemic}}]}$, where
the drip reaction \ref{rxn:drip} has probability $\Pr[\text{\ref{rxn:drip}}]\sim p(x-y)^2 \leq p(1-y)^2$ and the epidemic reaction \ref{rxn:i-1epidemic} has probability $\Pr[\text{\ref{rxn:i-1epidemic}}]\sim 2y(1-y)$. Assuming in the worst case that $y(t_{i}^{0.1}) = 0.1p$, then the number of interactions $T = (t_{i+1}^{0.1}-t_{i}^{0.1})n$ for $Y$ to increase from $0.1pn$ to $0.1n$ is a sum of independent geometric random variables with mean 
\begin{align*}
\E[T] &\geq \sum_{Y=0.1pn}^{0.1n - 1} \frac{1}{p(1 - Y/n)^2 + 2(Y/n)(1-Y/n)}
\sim n\int_{0.1p}^{0.1} \frac{dy}{p(1-y)^2 + 2y(1-y)}
\\
&= n\int_{0.001}^{0.1} \frac{dy}{(1-y)(0.01+(1.99)y)}
\geq 1.481n.
% = \frac{n}{2}\int_{0.01rp}^{0.9} \qty(\frac{1}{1-y} + \frac{2 - p}{p+(2-p)y})dy
% \\
% & = \frac{n}{2}\qty[-\ln(1-y) + \ln(p + (2-p)y)]_{0.01rp}^{0.9}
% \\
% & = \frac{n}{2}\qty[-\ln(0.1)+\ln(1.8+0.1p) + \ln(1 - 0.01rp) - \ln(p(1+0.02r - 0.01rp))]
% \\
% & \approx
% \frac{n}{2}\qty[-\ln(0.1)+\ln(1.8) +\frac{p}{18} - 0.01rp - \ln(p) -0.02r + 0.01rp]
% \\
% & \approx
% \frac{n}{2}\qty[2.89 + \frac{p}{18} + \ln(\frac{1}{p}) - 0.02r]
\end{align*}

Note that the probability in the geometric includes the term $p(1-y)^2 \geq 0.81p$ since $y\leq 0.1$, thus the minimum geometric probability $p^* \geq 0.81p$ is bounded by a constant. Also the number of terms in the sum is $\Theta(n)$, so by Corollary~\ref{cor:janson-wvhp}, with $\mu \geq 1.481n$,
$\Pr[T \leq 1.48 n] \leq \exp(-\Theta(n))$, so the time $t_{i+1}^{0.1}-t_{i}^{0.1} = T/n \geq 1.48$ with very high probability.
\end{proof}

Our main definition will refer to the times $t_i^{0.9}$ when the fraction reaches $0.9$, so we will need a bound the time it takes for $c_{\geq i}$ to increase from $0.1$ to $0.9$ by epidemic.
\begin{lemma}
\label{lem:clock-epidemic}
$t_i^{0.9} - t_i^{0.1}\leq 2.2$ with very high probability.
\end{lemma}

\begin{proof}
We can low bound $t_i^{0.9} - t_i^{0.1}$ by the time it takes for an epidemic to grow from a fraction $0.1n$ to $0.9n$. By Lemma~\ref{lem:epidemic}, this takes parallel time $t$, where
\[
\E[t]\sim\frac{\ln(0.9) - \ln(1 - 0.9) - \ln(0.1) + \ln(1-0.1)}{2} = \ln(9) < 2.2.
\]
Since $\ln(9)(1+\epsilon) < 2.2$, this completes within parallel time $2.2$ with very high probability.
\end{proof}

We will also use an upper bound on how long it takes the clock to move from one minute to the next.

\begin{lemma}
\label{lem:clock-upper-bound}
$t_{i+1}^{0.9}-t_{i}^{0.9}\leq 3.86$ with very high probability.
\end{lemma}

\begin{proof}
Define $x = x(t) = c_{\geq i}(t)$ and $y = y(t) = c_{> i}(t)$. For $t \geq t_i^{0.9}$, we have $x(t) \geq 0.9$.
The number of interactions for $Y = yn$ to increase by $1$ is a geometric random variable with mean $\frac{1}{\Pr[\text{\ref{rxn:drip}}] + \Pr[\text{\ref{rxn:i-1epidemic}}]}$, where the drip reaction \ref{rxn:drip} has probability $\Pr[\text{\ref{rxn:drip}}]\sim p(x-y)^2 \geq p(0.9-y)^2$ and the epidemic reaction \ref{rxn:i-1epidemic} has probability $\Pr[\text{\ref{rxn:i-1epidemic}}]\sim 2y(1-y)$. Assuming in the worst case that $y(t_{i}^{0.9}) = 0$, then the number of interactions $T = (t_{i+1}^{0.9}-t_{i}^{0.9})$ for $Y$ to increase from $0$ to $0.9n$ is a sum of independent geometric random variables with mean 
\begin{align*}
\E(T) &\leq \sum_{Y=0}^{0.9n - 1} \frac{1}{p(0.9 - Y/n)^2 + 2(Y/n)(1-Y/n)}
\sim n\int_{0}^{0.9} \frac{dy}{p(0.9-y)^2 + 2y(1-y)}
\\
& = 
n\int_{0}^{0.9} \frac{dy}{0.01(0.9-y)^2 + 2y(1-y)}
\leq 3.856 n.
\end{align*}

When $y<0.1$ we have $\Pr[\text{\ref{rxn:drip}}] \geq 0.64p$ and when $0.1 \leq y \leq 0.9$ we have $\Pr[\text{\ref{rxn:i-1epidemic}}] \geq 0.18$, so the minimum geometric probability $p^* \geq 0.64p$ is bounded by a constant. Also the number of terms in the sum is $\Theta(n)$, so by Corollary~\ref{cor:janson-wvhp}, with $\mu \leq 3.856n$,
$\Pr[T \geq 3.86 n] \leq \exp(-\Theta(n))$, so the time $t_{i+1}^{0.9}-t_{i}^{0.9} = T/n \leq 3.86$ with very high probability.
\end{proof}

We can now combine the previous lemmas to get a main theorem concerning the behavior of the clock.
For a clock agent $a$, define $a.\fieldhour = \floor{\frac{a.\fieldminute}{k}}$.
Define $\hourstart_h = \min\big(t: |\{a:a(t).\fieldhour \geq h\}| \geq 0.9|\clocks| \big)$ be the first time when the fraction of clock agents at hour $h$ or beyond reaches $0.9$ and $\hourend_h = \min\big(t: |\{a:a(t).\fieldhour > h\}| \leq 0.001|\clocks|\big)$ be the first time when the fraction of clock agents beyond hour $h$ reaches $0.001$. 
Define the \emph{synchronous hour h} to be the parallel time interval 
$[\hourstart_h, \hourend_h]$, 
i.e. when fewer than 0.1\%  are in any hour beyond $h$ and at least (90 - 0.1) = 89.9\% are in hour $h$. Note that if $\hourend_h < \hourstart_h$ then this interval is empty, but we show this happens with low probability.
Recall $c = |\clocks|/n$ is the fraction of clock agents and
 $k = \kconstant$ is the number of minutes per hour.

\begin{theorem}
\label{thm:clock}
Let $j \in \{1,\ldots,k-1\}$.
For every synchronous hour $h$, its length $\emph{\hourend}_h - \emph{\hourstart}_h \geq [1.48(k-j) - 2.2]/c^2$ with probability $1-O(1/n^{0.7j})$. 
The time between consecutive synchronous hours $\emph{\hourstart}_{h-1} - \emph{\hourstart}_h < 3.86k / c^2$ with very high probability.
\end{theorem}

\begin{proof}
Note that the previous lemmas assumed $|\clocks| = n$, so the entire population was running the clock algorithm. In reality, we have a fraction $c = |\clocks| / n$ of clock agents. The reactions we considered only happen between two clock agents, which interact with probability $\sim c^2$. Thus we can simply multiply the bounds from our lemmas by the factor $\frac{1}{c^2}$ to account for the number of regular interactions for the requisite number of clock interactions to happen, which is very close to its mean with very high probability by standard Chernoff bounds.

Since $c.\fieldhour = h \iff hk \leq c.\fieldminute < (h+1)k$, the time
$\hourstart_h = t_{h k}^{0.9}$ and $\hourstart_{h+1}=t_{(h+1) k}^{0.9}$ For the upper bound, by Lemma~\ref{lem:clock-upper-bound} we have $t_{i+1}^{0.9}-t_{i}^{0.9}\leq 3.86 / c^2$ with very high probability. Summing over the $k$ minutes in hour $h$ gives $\hourstart_{h+1} - \hourstart_h < 3.86k / c^2$ with very high probability.

For the lower bound, we first consider the number of non-leaky minutes among the $k$ minutes in hour $h$. By Lemma~\ref{lem:clock-early-drip}, each minute has an independent probability $O(1/n^{0.7})$ of being leaky. Thus with probability $1-O(1/n^{0.7j})$ we have less than $j$ leaky minutes for each $j=1, \ldots, k$, so the number of non-leaky minutes is at least $k-j+1$.

We will reason about the interval from $t_{hk}^{0.1}$ to $t_{i}^{0.1}$, where $i$ is the largest non-leaky minute in hour $h$. Now we can apply Lemma~\ref{lem:clock-lower-bound} $k-j$ times for each non-leaky minute before $i$ to conclude that $t_{i}^{0.1} - t_{hk}^{0.1} \geq 1.48(k-j)/c^2$ with very high probability. Since minute $i$ is also non-leaky, we can apply Lemma~\ref{lem:clock-level-gap} to conclude $c_{> i}(t_{i}^{0.1})<0.001c$. Since the count beyond minute $i$ is still very small at time $t_{i}^{0.1}$, we have $t_{i}^{0.1} \leq \hourend_h$. Finally, we must actually start the argument at time $t_{hk}^{0.9}$, which is after time $t_{hk}^{0.1}$. By Lemma~\ref{lem:clock-epidemic} we have $\hourstart_h = t_{hk}^{0.9} - t_{hk}^{0.1} \leq 2.2/c^2$ with very high probability, so we conclude that 
$\hourend_h - \hourstart_h \geq [1.48(k-j) - 2.2]/c^2$.
\end{proof}

Since every hour takes constant time with very high probability, all $L$ hours will finish within $O(\log n)$ time.
In this paper, we will set $p = 0.01$, $k = \kconstant$ and $j = 2$ to give us sufficiently long synchronous hours with sufficiently high probability $(1 - O(1/n^{1.4})$ for later proofs. As with all our high probability claims, tuning these constants can make this polynomial factor in Theorem~\ref{thm:clock} higher, and make the synchronous hours longer to make later high probability proofs tighter. Also most of our simulations in Section~\ref{sec:simulation}

We next discuss how the main result of Theorem~\ref{thm:clock} changes with parameters $p$ and $k$. The lower bound constant $1.48$ coming from Lemma~\ref{lem:clock-lower-bound} and upper bound constant $3.86$ coming from Lemma~\ref{lem:clock-upper-bound} depend on the value $p = 0.01$. These constants will scale will $\log(\frac{1}{p})$, as shown in Figure~\ref{fig:clock-constants}. So by making $p$ smaller, the relative distance between the constants gets tighter.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/bound_constants.pdf}
    \caption{
    Generalizing the lower and upper bound constants from Theorem~\ref{thm:clock},
    indicating the probable length of each synchronous hour in units of parallel time,
    based on setting alternate values of the drip reaction probability $p$.
    Theorem~\ref{thm:clock} uses constants $1.48$ and $3.86$ for $p = 0.01$. These bounds come from numerically integrating the integrals used in Lemma~\ref{lem:clock-lower-bound} and Lemma~\ref{lem:clock-upper-bound} for varying values of $p$.
    }
    \label{fig:clock-constants}
\end{figure}

Figure~\ref{fig:hour-length-varying-p} shows average synchronous hour lengths from simulation, at the fixed value $k = 5$, varying $p$, along with the predicting lower and upper bounds from generalizing Theorem~\ref{thm:clock} to use the constants in Figure~\ref{fig:clock-constants} with $k = 5$. Note our upper bound in Theorem~\ref{thm:clock} is on the length between consecutive synchronous hours, which in turn is an upper bound on the length within each synchronous hour.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/hour_length_varying_p.pdf}
    \caption{
    The average length of a synchronous hour when $k = 5$ and $p$ is varied, when the entire population are $\roleclock$ ($c=1$). For each population size $n$, the lengths of each synchronous hour across 20 simulated trials were calculated and averaged. If $n$ is too small compared to $p$, the time exceeds the upper bound. This is because the upper bound holds for the limit of large $n$, when we can assume the number of drip reactions is proportional to the small but positive dripping rate $px^2$. When $n$ is too small, we must wait longer (in parallel time) to be sure to see the earliest drip reactions.
    }
    \label{fig:hour-length-varying-p}
\end{figure}

The length of an hour scales linearly with $k$, as we would expect. Figure~\ref{fig:hour-length-varying-k} shows average synchronous hour lengths from simulation, at our fixed value of $p = 0.01$, varying $k$ and population size $n$. We see the constant from simulation is about $2.3$.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/hour_length_varying_k.pdf}
    \caption{
    The average length of a synchronous hour when $p = 0.01$ and $k$ is varied, when the entire population are $\roleclock$ ($c=1$). For each population size $n$, the lengths of each synchronous hour across 20 simulated trials were calculated and averaged.
    }
    \label{fig:hour-length-varying-k}
\end{figure}


We finally show one more lemma concerning how the $\roleclock$ agents affect the $\rolemain$ agents.
The $\roleclock$ agents will change the $\fieldTlevel$ of the $\unbiased$ agents via line~\ref{line:clock-update-reaction} of \phaseMainAveraging. There are a small fraction $0.001|\clocks|$ of $\roleclock$ agents that might be running too fast and thus have a larger $\fieldhour$ than the synchronized hour. We must now show these agents are only able to affect a small fraction of the $\rolemain$ agents. Intuitively, the $\roleclock$ agents with $\fieldhour > h$ bring up the hour of both $\unbiased$ agents and other $\roleclock$ agents. The following lemma will show they don't affect too many $\rolemain$ agents before also bringing in a large number of $\roleclock$ agents, a similar result to Lemma 8 in \cite{gasieniec2020time}.

We will redefine $c_{> h} = c_{> h}(t) = |\{c:c.\fieldhour > h\}| / |\clocks|$ to be the fraction of $\roleclock$ agents beyond hour $h$, and similarly $m_{>h} = m_{>h}(t) = |\{m:m.\fieldhour > h\}| / |\mains|$ to be the fraction of $\rolemain$ agents beyond hour $h$. 


\begin{lemma}
\label{lem:mains-small-hour}
For all times $t \leq \hourend_h$, we have
$m_{>h}(t) \leq 1.2 c_{> h}(\hourend_h) = 0.0012$ with very high probability.
\end{lemma}

\begin{proof}
We have $c_{>h}(\hourend_h) = 0.001$ by the definition of synchronous hour $h$.
Thus it suffices to show that $m_{>h}(t) \leq 1.2 c_{> h}(\emph{\hourend}_h)$.

Recall $c = |\clocks| / n$ and $m = |\mains| / n$, 
so $c \cdot c_{>h}$ and $m \cdot m_{>h}$ are rescaled to be fractions of the whole population. 

We will assume in the worst case that every $\rolemain$ agent can participate in the clock update reaction
\[
C_h, M_j \to C_h, M_h \text{ where } h > j,
\]
so the probability of clock update reaction is $2 c \cdot c_{>h} \cdot m(1-m_{>h})$.
Among the $\roleclock$ agents, we will now only consider the epidemic reactions $C_h, C_j \to C_h, C_h$ between agents in different hours $h > j$, so the probability of the clock epidemic reaction is $2 c^2 \cdot c_{>h}(1-c_{>h})$.

We use the potential $\Phi(t) = m_{> h}(t) - 1.1\cdot c_{> h}(t)$. Note that initially $\Phi(0) = 0$ since both terms are $0$. The desired inequality is $\Phi(\hourend_h) \leq 0.1c_{>h}(\hourend_h) = 0.0001$, and we will show this holds with very high probability by Azuma's Inequality because $\Phi$ is a supermartingale. The clock update reaction increases $\Phi$ by $\frac{1}{|\mains|} = \frac{1}{mn}$. The clock epidemic reaction decreases $\Phi$ by $\frac{1.1}{|\clocks|} = \frac{1.1}{cn}$. This gives an expected change
\begin{align*}
\E[\Phi(t+1/n)-\Phi(t)] &= \frac{1}{mn}\qty [ 2 c \cdot c_{>h} \cdot m(1-m_{>h})] - \frac{1.1}{cn}\qty [ 2 c^2 \cdot c_{>h}(1-c_{>h})]
\\
& = \frac{2c \cdot c_{>h}}{n}\qty[(1-m_{> h}) - 1.1(1- c_{>h})]
\\
& \leq \frac{2c \cdot c_{\geq i}}{n}\qty[1 - 1.1(0.999)] < 0.
\end{align*}

Thus the sequence $\big(\Phi_j = \Phi(\frac{j}{n})\big)_{j=0}^{n \cdot \hourend_h}$ is a supermartingale, with bounded differences
$|\Phi_{j+1}-\Phi_j| \leq 
\max\qty(\frac{1}{mn}, \frac{r}{cn}) =
O(\frac{1}{n})$. 
So we can apply Azuma's Inequality (Theorem~\ref{thm:azuma}) to conclude
\[
\Pr[\Phi_{n \cdot \hourend_h} \geq \delta] \leq \exp \qty(-\frac{\delta^2}{2\sum_{j=0}^{n \cdot \hourend_h} O(\frac{1}{n})^2})
= \exp(-O(n)\delta^2),
\]
since by Theorem~\ref{thm:clock}, we have time $\hourend_h = O(1)$ with very high probability. Thus we can choose $\delta = 0.1c_{>h}(\hourend_h) = 0.0001$ to conclude that $m_{>h}(\hourend_h) \leq 1.2c_{>h}(\hourend_h)$ with very high probability $1 - \exp(-\Omega(n)) = 1 - O(n^{-\omega(1)})$.

The lemma statement for times $t \leq \hourend_h$ simply follows from the monotonicity of the value $m_{>h}$, since agents only decrease their $\fieldhour$ field.
\end{proof}

